Compressed spectral screening for large-scale differential correlation analysis with application in selecting Glioblastoma gene modules

Differential co-expression analysis has been widely applied by scientists in understanding the biological mechanisms of diseases. However, the unknown differential patterns are often complicated; thus, models based on simplified parametric assumptions can be ineffective in identifying the differences. Meanwhile, the gene expression data involved in such analysis are in extremely high dimensions by nature, whose correlation matrices may not even be computable. Such a large scale seriously limits the application of most well-studied statistical methods. This paper introduces a simple yet powerful approach to the differential correlation analysis problem called compressed spectral screening. By leveraging spectral structures and random sampling techniques, our approach could achieve a highly accurate screening of features with complicated differential patterns while maintaining the scalability to analyze correlation matrices of $10^4$--$10^5$ variables within a few minutes on a standard personal computer. We have applied this screening approach in comparing a TCGA data set about Glioblastoma with normal subjects. Our analysis successfully identifies multiple functional modules of genes that exhibit different co-expression patterns. The findings reveal new insights about Glioblastoma's evolving mechanism. The validity of our approach is also justified by a theoretical analysis, showing that the compressed spectral analysis can achieve variable screening consistency.

==> intro_old.tex <==
\subsection{Motivating application and the data set} \label{sec:dataset}

RNA sequencing (RNA-seq) is a powerful tool used in genomics to quantify the abundance of mRNA transcripts in a sample. Such data can be used to compare one sample to another to identify differences that contribute to specific biological and clinical phenomena. For example, differential expression analyses can be used to compare tumor samples to normal tissue samples in order to identify mRNA transcripts with differing abundances. This helps to identify targets for downstream study with more specified purposes. \citep{krupp2012rna,lonsdale2013genotype,wan2015bioxpress,li2016cancer}.

%One of the major drawbacks of differential expression analysis is that it can suffer from batch effect due to differences in how the samples were processed prior to being sequenced. This issue is particularly relevant when one set of samples are generated using one processing protocol and another set of samples are derived using a separate processing protocol. This issue can be rectified through normalization if there are overlapping samples between the two datasets \citep{li2016cancer,danielsson2015assessing,fernandez2016oasis,wang2018unifying}.

The Cancer Genome Atlas (TCGA) is a large collection of tumor and normal tissue samples collected from over 10,000 patients that catalogued the molecular abnormalities seen across 33 separate cancer types \citep{cancer2015comprehensive}. The Genotype Tissue Expression (GTEx) project is another large-scale sequencing project that processed over 9,000 samples from 53 different tissues from over 500 healthy individuals \citep{lonsdale2013genotype,gtex2015genotype,wang2018unifying}. The study identified differentially expressed genes across multiple tumor types using differential expression analysis by comparing the tumor samples from TCGA to the normal tissue samples from GTEx, after batch effects correction. However,  gliomas were excluded from the GTEx analysis because TCGA did not sequence a sufficient number of normal brain samples for the type of analysis \citep{wang2018unifying}. In addition, normalization in studying the gliomas are not available, rendering the standard differential expression analysis infeasible. The proposed approach in this paper focus on the differential  pattern on correlation instead of the expression levels. Therefore, our method can serve as an alternative of the traditional differential analysis to identify meaningful differential patterns when normalization is not available, such as in the case of analyzing gliomas.

Gliomas are highly invasive primary brain tumors that are challenging to neurosurgically resect without significant patient morbidity.
 Approximately 20,000 patients are diagnosed with gliomas each year in the United States. Gliomas can be divided into several grades according the severity. Grade II and grade III gliomas are also known as lower grade gliomas, while grade IV gliomas are also known as glioblastoma multiforme.
 Glioblastoma multiforme is highly lethal and has a five year survival rate of less than 5\%. Although lower grade gliomas do not progress as fast as glioblastoma multiforme, they are also essentially uniformly lethal and can progress to glioblastoma multiforme. The median survival rate for lower grade gliomas is seven years. Lower grade gliomas and glioblastoma multiforme are typically managed surgically followed by chemotherapy and radiation therapy \citep{cancer2015comprehensive, bauman2009adult,yan2012molecular,louis20162016}. The 2016 World Health Organization’s guidelines for brain tumors now suggests that the classification of gliomas should be based on molecular characteristics instead \citep{louis20162016}. Given the recent recognition of the importance of molecular characteristics in the classification of gliomas and the lethality of these tumors, it is crucial to identify genes of interest that could be studied further by the field. We compare the glioblastoma multiforme samples from the TCGA dataset  to the normal brain samples from the GTEx dataset using the approach described in this paper. Given that the lower grade gliomas (grade II or III) have a better prognosis than glioblastoma multiforme (a grade IV glioma) but can ultimately progress to glioblastoma multiforme, we hypothesize that lower grade gliomas would show an intermediate level of dysregulation between glioblastoma multiforme and normal brain tissue and use the lower grade gliomas a validation set for this study, as suggested in many other studies \citep{lonsdale2013genotype, cancer2015comprehensive, gtex2015genotype, yan2012molecular,louis20162016}. The key challenge in this setting comes from the dimensionality of the problem. We have a few hundreds observations on 51,448 genes. The calculation of all correlation coefficients between so many genes is infeasible. Let alone an in-depth differential analysis. Even if basic filtering is applied, there are still too many for a computationally feasible analysis. Our method is designed to handle the differential correlation analysis in such large-scale problems.  The detailed analysis is described in Section~\ref{sec:data-analysis}.


